Spatial Positioning Token (SPToken) for Smart Parking

In this paper, we describe an approach to guide drivers searching for a parking space (PS). The proposed system suggests a sequence of routes that drivers should traverse in order to maximise the expected likelihood of finding a PS and minimise the travel distance. This system is built on our recent architecture SPToken, which combines both Distributed Ledger Technology (DLT) and Reinforcement Learning (RL) to realise a system for the estimation of an unknown distribution without disturbing the environment. For this, we use a number of virtual tokens that are passed from vehicle to vehicle to enable a massively parallelised RL system that estimates the best route for a given origin-destination (OD) pair, using crowdsourced information from participant vehicles. Additionally, a moving window with reward memory mechanism is included to better cope with non-stationary environments. Simulation results are given to illustrate the efficacy of our system.

==> 03_01_long_path_problem.tex <==
% LONGEST PATH PROBLEM -----------------------------------------------------------------------------------
\mytodo{
Roman: Bellman-Fords, Johnson, Dijkstra, First Depth Search, negative edges, cycles.
}
% LONGEST PATH PROBLEM -----------------------------------------------------------------------------------


==> 03_02_multi_obj_optimization.tex <==
% MULTI_OBJECTIVE OPTIMIZATION ---------------------------------------------------------------------------
\mytodo{
Rodrigo, Sergiy: If linear combination all the above, Pareto front, others.
}

The preferences of drivers are considered in the proposed framework. For example, some drivers favour 
shorter travel distances over larger numbers of parking spots while others are just opposed. Thus, 
a weight can be chosen by a driver and assigned to the corresponding cost in the objective function.
% MULTI_OBJECTIVE OPTIMIZATION ---------------------------------------------------------------------------

